Measurement of the branching fraction for the decay Upsilon(4S) -> Upsilon(1S)pi+pi-

We study transitions between Upsilon states with the emission of charged pions using 604.6/fb of data collected with the Belle detector at the KEKB asymmetric-energy e+e- collider. The measured product branching fraction is B(Upsilon(4S) -> Upsilon(1S)pi+pi-) * B(Upsilon(1S) -> mu+mu-) = = (2.11 +/- 0.30(stat.) +/- 0.14(sys.))*10^(-6) and the partial decay width is Gamma(Upsilon(4S) -> Upsilon(1S)pi+pi-) = = (1.75 +/- 0.25(stat.) +/- 0.24(sys.)) keV.

==> u4u1_hepex_2_abstract.tex <==
We study transitions between Upsilon states with the emission of
charged pions using 604.6/fb of data collected
with the Belle detector at the KEKB asymmetric-energy e+e- collider.
The measured product branching fraction is
B(Upsilon(4S) -> Upsilon(1S)pi+pi-) * B(Upsilon(1S) -> mu+mu-) =
 (2.11 +/- 0.30(stat.) +/- 0.14(sys.))*10^(-6)
and the partial decay width is
Gamma(Upsilon(4S) -> \Upsilon(1S)pi+pi-) = 
 (1.75 +/- 0.25(stat.) +/- 0.24(sys.)) keV.

